Variational Distillation of Diffusion Policies into Mixture of Experts

This work introduces Variational Diffusion Distillation (VDD), a novel method that distills denoising diffusion policies into Mixtures of Experts (MoE) through variational inference. Diffusion Models are the current state-of-the-art in generative modeling due to their exceptional ability to accurately learn and represent complex, multi-modal distributions. This ability allows Diffusion Models to replicate the inherent diversity in human behavior, making them the preferred models in behavior learning such as Learning from Human Demonstrations (LfD). However, diffusion models come with some drawbacks, including the intractability of likelihoods and long inference times due to their iterative sampling process. The inference times, in particular, pose a significant challenge to real-time applications such as robot control. In contrast, MoEs effectively address the aforementioned issues while retaining the ability to represent complex distributions but are notoriously difficult to train. VDD is the first method that distills pre-trained diffusion models into MoE models, and hence, combines the expressiveness of Diffusion Models with the benefits of Mixture Models. Specifically, VDD leverages a decompositional upper bound of the variational objective that allows the training of each expert separately, resulting in a robust optimization scheme for MoEs. VDD demonstrates across nine complex behavior learning tasks, that it is able to: i) accurately distill complex distributions learned by the diffusion model, ii) outperform existing state-of-the-art distillation methods, and iii) surpass conventional methods for training MoE.

==> Contents/Experiments.tex <==
\section{Experiments}
Our experiments aim to answer the following key questions: i) Can \acrshort{method} replicate the performance and diversity of Diffusion models that it distills? ii) How is the performance of \acrshort{method} compared to SoTA MoE training methods? iii) How is the inference speed of \acrshort{method} compared to the original diffusion models? iv) How do the key hyperparameters influence the final performance of \acrshort{method}? 
To answer these questions, we conducted experiments on \textbf{nine} challenging behavior-learning tasks with history observations, including \textbf{two} tasks with image observations.
\input{Figs/distillation_1}

\subsection{Baselines}
To show that \acrshort{method} is capable of distilling different diffusion models but not specially designed for a specific model, we distill one discrete score-based diffusion model (\textbf{DDPM}) \cite{ho2020denoising} \todo{TODO: Maybe also mention what sampler do we use} and one continuous score-based diffusion model (\textbf{BESO}) \cite{song2020score, reuss2023goal} \todo{TODO: The same, what sampler here}. We compare the performance of \acrshort{method} against the original diffusion models and their one-step variants(referred as \textbf{DD-1} and \textbf{CD-1} in figures), where only one denoising step is applied during inference. We also compare the performance of \acrshort{method} with the Consistency Model (\textbf{CM}) \cite{song2023consistency}, which is the SoTA diffusion distillation method. In our evaluation, we applied CM on the same continuous diffusion model as \acrshort{method}-CD used. At the end, we also compare the performance against two SoTA \acrshort{moe} training algorithms, Expecation-Maximization (EM) \todo{CITE} and Information Maximizing Curriculum (IMC) \cite{blessing2024information}. In order to make EM and IMC stronger baselines and prevent the advantages introduced by different model architectures, we augmented them with a similar transformer backbone that we used in \acrshort{method}. We renamed the augmented algorithm as \textbf{EM-GPT} and \textbf{IMC-GPT}, respectively.

\subsection{Environments}
We conducted experiments on 9 challenging robot manipulation tasks, seven of them come from the D3IL dataset \cite{jia2024towards}, one relay kitchen task environment\cite{gupta2019relay}, and one robot block-push task\cite{florence2022implicit, reuss2023goal}.
\paragraph{D3IL Datasets.} 
Datasets with Diverse Human Demonstrations for Imitation Learning (D3IL) \cite{jia2024towards} is a recently proposed dataset designed explicitly to evaluate the model's ability to learn multi-modal behavior. The datasets consist of several challenging robot manipulation tasks using Franka. We chose five representative state-based tasks (avoiding, aligning, pushing, stacking-1, and stacking-2) and two image-based tasks (image-based sorting and stacking). More importantly, D3IL datasets provide \textbf{task entropy}, a measure to quantify the diversity of model behavior that an agent learned, which ranges from 0 to 1 for all the tasks, higher task entropy indicates the policy is better at capturing the diversity in demonstration. We provide an in-detailed task description and explanation of task entropy in Appendix B. \todo{TODO: Add appendix and put reference here} 
\paragraph{Relay Kitchen Environment.} 
A multi-task kitchen environment with long-horizon manipulation tasks such as moving kettle, open door, and turn on/off lights. The dataset consists of 566 human-collected trajectories with sequences of 4 executed skills. We used the same experiment settings and the pretrained diffusion models from \cite{reuss2023goal}. For each seed we conducted 100 rollouts. 

\paragraph{XArm Block Push Environment.}

% We used the adapted goal-conditioned variant. The Block-Push Environment consists of an XARm robot that must push two blocks, a red and a green one, into a red and green squared target area. The dataset consists of 1000 demonstrations collected by a deterministic controller with 4 possible goal configurations. The methods got 0.5 credit for every block pushed into one of the targets with a maximum score of 1.0.
% (\todo{TODO: adapt, currently copy-paste from beso})
\subsection{Distillation Performance}
We compare the distillation performance of \acrshort{method} against Consistency Model and 1-step version of the diffusion model, the results are presented in Figure \ref{fig:distillation_1} and Figure \ref{fig:distillation_2}. The results for consistency models and \acrshort{method} are reported in mean and standard deviation across 4 random seed, while .From the results we observed several interesting findings: i) 1-step continous-time diffusion policies (CD-1) are actually strong baselines in behaviour learning tasks, previous works \todo{add some citation here} mentioned these types of diffusion models are able to generate high-quality samples with less denoising steps but the 1-step performance were rarely discussed. ii) in most of the task, \acrshort{method} is able to replicate the performance from the original diffusion model, and the distillation performance is comparable if not better than Consistency Model. The only exception seems to be the Aligning task, where Consistency Model achieved higher success rate than \acrshort{method}-CD. However, \acrshort{method}-CD still demonstrated higher entropy in this task, which indicates the policies learns more versatile ways to solve this task. iii) in some tasks, we observed \acrshort{method} achieved higher success rate than original diffusion models, e.g., Aligning, Pushing, image-based Sorting and image-based Stacking. We attribute this into two reasons, first, in tasks where \acrshort{method} achieved lower entropy than the original diffusion models, the model learned less versatile skills from the diffusion model, leading in repeatly execution of similar skill, which results in higher success rate. This pattern is also observed in Pushing task, where 1-step continuous-time diffusion achieved higher success rate than the default setting with 16 denoising steps. This pattern will be further discussed in the ablation study, where \acrshort{method} with 1 components achieves highest success rate while possessing 0 entropy. In image-based sorting and stacking tasks, \acrshort{method}-CD achieves higher success rate and entropy than the original diffusion model, we attribute this to the limited amount of denosing steps that diffusion takes.

\input{Figs/distillation_2}
% \todo{Todo: kick the table into appendix}
% \input{Tables/main_results}
\subsection{Comparison with MoE learning from scratch}
We compared distilled \acrshort{moe} policies with other \acrshort{moe} training methods. The results in \todo{add ref to table 1}show \acrshort{method} can consistently outperform these method across all the tasks in terms of both success rate and task entropy. We attribute that to the great generalization ability of pre-trained score function and the stable update provided by our decompositional objective. To clarify the huge performance gap in vision-based tasks, here for \acrshort{method}, we copy the vision encoder from pretrained diffusion models, which is considered a widely applied technique for distillation methods. For the hyperparameter setting we use the same network architecutre for all four methods, and sweep over keep hyperparameters via a grid search, for details of the grid search and optimal hyperparameters please refer to Appendix \todo{REF Appendix}. 
\input{Tables/moe_results}
% \input{Tables/main_results}
\subsection{Inference Times}
\input{Tables/inference_time_double_tables}
In this section, we aim to answer the question iii) Is \acrshort{method} significantly faster than original diffusion models in inference? To avoid advantages brought by utilizing simpler network architecture, we use similar transformer backbone with identical number of layers and heads in this evaluation. The data in \todo{Add Table Reference} reflects the average results from 200 predictions. All evaluations were performed on a system equipped with an RTX 3070 GPU and an Intel i7-12700 CPU. The results are reported in both Number of Function Evaluations (NFE) and absolute inference time (in milliseconds).
We conducted the evaluation in an state-based task (avoiding) and an image-based task (pushing). The results suggest that \acrshort{method} is significantly faster than the original diffusion models in both cases, even when the diffusion model only takes one deniosing step.

\subsection{Ablation Studies}
\input{Figs/results/ablation_study/Ablation_all}
% \input{Figs/results/ablation_study/num_cmps_success}
In this section, we evaluate how key design choices influence the performance of \acrshort{method}. First we evaluate the influence of the number of components. We conducted experiments on avoiding environment, we kept all the hyperparameters but number of components identical across all runs, the results are reported in Figure \ref{ablation:num_cmps} with average values across four seeds. When number of components equals 1, \acrshort{moe} is equivalent to an uni-mode Gaussian policy, which is unable to capture the multi-modes action distribution from the diffusion model, resulting in 0 task entropy. It is not surprise in this case the success rate is higher as the policy keeps following the same path at every rollouts.

% \input{Figs/results/ablation_study/gating}
Next we evaluate the design choice of learning the state-dependent gating distribution as a parameterized network $q^{\xi}(z|\bm{s})$ or using a state-independent uniform gating $q(z)=1/N$, where $N$ is the number of components. We conducts experiments on three state-based tasks: avoiding, aligning and stacking. The results in Figure \ref{fig:main_figure} show that learning gating improves the success rate in all three tasks. In the other hand, using uniform gating improve the entropy in avoiding and stacking. This is because in the uniform gating cases, each expert are treated equally in every state during both training and evaluation, so each expert must be good at every state, while state-dependent gating allows expert to specialize at different state. \todo{repharse the sentences}

% \input{Figs/results/ablation_study/sampling_strategy}
In the end we evaluate how different nosie level sampling strategies in training influence the final model performance. The experiments are conducted in the avoiding task. Four sampling strategies are evaluated: \textbf{min} refers to only use the score from minimum noise level $\sigma_{\min}$, \textbf{max} refers use the score from max noise level $\sigma_{\max}$, \textbf{uniform} refers to draw noise level from a uniform distribution $\sigma \sim U(\sigma_{\min}, \sigma_{\max})$ for each sample, \textbf{interval} sampling also sample noise from a uniform distribution but the lower bound and higher bound of sampling intervals are hyperparameters to be determined. Results in Figure \ref{ablation:sigma_sampling} show that interval sampling achieves highest success rate among other methods. Interval sampling works the best in practice so we keep it as default setting in our experiments.

==> Contents/Limitations.tex <==
\section{Limitations}
Although this work primarily concentrates on distilling behaviors, VDD is not straightforwardly applicable to generating very high-dimensional data like images due to the \acrshort{moe}'s contextual mean and covariance prediction. Scaling VDD to images requires further extensions like prediction in a latent space. We consider this extension as an interesting future work. 
Additionally, the number of experts needs to be pre-defined by the user. As the ablations show, having a high number of experts does not harm VDD's training and performance and is therefore not considered a crucial hyperparameter. However, a redundantly high number of experts could potentially decrease the usage in post hoc fine-tuning using reinforcement learning. 


% We noticed two main limitations of the proposed method. First is the applicability to tasks with high-dimensional action space (e.g., image generation, control of humanoid robots, etc) is not verified, as learning contextual high-dimensional Gaussian (especially with full covariance) is notoriously unstable. The second limitation is the expressiveness of \acrshort{moe} relies on number of components, in order to distill more complex policies we might need to use more components, which could potentially increase the computational cost in both training and inference.

% Hard to scale to high-dimensional tasks (learning GMM for image tasks would be very difficult), However, it could be possible if we do image generation in a lower dimensional latent space? The noise level needed to be hand chosen.

==> Contents/Methods.tex <==
\section{Distilling GMM from Diffusion Models}
\subsection{Variational Inference Components Updates}
Problem Formulation

\begin{align}
    \theta^* = \arg\min_\theta \int_s\text{KL}(q(x|s;\theta)||D(x|s))ds
\end{align}

Decompose the objective for each component (cite VIPS) 
\begin{align*} 
J(\theta) =& -\int_s \int_x q(x|s;\theta)\log\frac{q(x|s;\theta)}{D(x|s)}dxds \\=&\int_s\int_x \sum_o q(o|s)q(x|o,s)[\log D(x|s)- \log q(x|s)]dxds \\=&\int_s \sum_o q(o|s) \int_x q(x|o,s)[\log D(x|s)-\log q(o|s)-\log q(x|o,s) \\&+ \log q(o|x,s)]dxds \\ =&\int_s \sum_o q(o|s)[\int_x q(x|o,s)[\log D(x|s)+\log q(o|x,s))dx+H(q(x|o,s)]] \\ &+ H(q(o|s)) ds 
\end{align*}

Objective for each component
\begin{align}
J_o(\theta)=\mathbb{E}_{s\sim p(s)}[\mathbb{E}_{x\sim q(x|s,o;\theta)}[\log D(x|s)+\log \tilde{q}(o|x,s)]+H[q(x|s,o;\theta)]]
\end{align}

Reparametrization Trick
\begin{align*}
\nabla_\theta J^1_o(\theta) &= \nabla_\theta \mathbb{E}_s \mathbb{E}_{\epsilon \sim N(0, I)}[\log D(h_\theta(\epsilon,s)|s)+\log \tilde{q}(o|h_\theta(\epsilon,s),s)] \\&= \mathbb{E}_s\mathbb{E}_{\epsilon \sim N(0, I)}[\frac{\partial \log D(h_\theta(\epsilon,s)|s)}{\partial h_\theta(\epsilon,s)}\frac{\partial h_\theta(\epsilon,s)}{\partial \theta} \\&\quad\quad\quad +\frac{\partial \log \tilde{q}(o|h_\theta(\epsilon,s),s)}{\partial h_\theta(\epsilon,s)}\frac{\partial h_\theta(\epsilon,s)}{\partial \theta}] \\ &= \mathbb{E}_s\mathbb{E}_{\epsilon \sim N(0,I)}[F_{score}(h_\theta(\epsilon,s),s)\frac{\partial h_\theta(\epsilon)}{\partial \theta}\\&\quad\quad\quad+\frac{\partial \log \tilde{q}(o|h_\theta(\epsilon,s),s)}{\partial h_\theta(\epsilon,s)}\frac{\partial h_\theta(\epsilon,s)}{\partial \theta}]
\end{align*} 

The learning objective for each component:
\begin{align*}
L = -\mathbb{E}
_{s\sim p(s)}[\mathbb{E}_{\epsilon\sim N(0, I)}[F_{score}(h(\epsilon, s),s)h_\theta(\epsilon, s)+\log \tilde{q}(o|h(\epsilon, s),s)]+H[q(x|s,o;\theta)]]
\end{align*}
\subsection{Recursive Gating Update}
Explain why we cannot update the Gating using VIPS: Need log-probability but we only have access to the gradient of log-probability.
Inspired by E-Step from EM algorithm:
\begin{align*}
    p_{\text{target}}(o|s)= \int p(a)p(o|a,s) da= \mathbb{E}_{a\sim p(a)} \left[\frac{p(a|s,o) p_{\theta'}(o|s)}{\sum_o p (a|s,o) p_{\theta'}(o|s)} \right]
\end{align*}
where $\theta'$ is the parameter of gating network from last step. The gating network $p_\theta(o|s)$ can be updated by minimize the Cross Entropy objective
\begin{align*}
    J_{\theta} = -\sum_o p_{\text{target}}(o|s)\log p_\theta(o|s)
\end{align*}
\subsection{Gaussian Mixture Models with History}
Needs some plots here

==> Contents/Structure.tex <==
\section{Structure of the Paper}
\subsection{Introduction}
\subsection{Related Work}
\begin{itemize}
    \item Diffusion Policies for Behavior Learning
    \item Mixture of Experts for Behavior Learning
    \item Distillation Methods for Diffusion Models
\end{itemize}
\subsection{Preliminaries}
\begin{itemize}
    \item Score-based Diffusion Policies for Behavior Learning
    \item Variational Inference
    \item Gaussian Mixture of Experts Models
\end{itemize}
\subsection{Variational Distillation of Score-Based Diffusion Models}
\begin{itemize}
    \item Introduce the (amortized) objective without introducing a model class 
    \item Introduce the objective for a Gaussian variational distribution. Mention limitations. Show visualizations.
    \item Extend the objective to Gaussian mixture models
\end{itemize}
\subsection{Experiments}
\subsection{Conclusion}

==> Figs/distillation_1.tex <==
\begin{figure}[!t]
    \scriptsize
    \centering
    \sloppy
    \begin{subfigure}{0.24\textwidth}
    \centering
    \input{Figs/results/success_rate/avoiding_success}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
    \centering
    \input{Figs/results/success_rate/aligning_success}
    \end{subfigure}
    % \hspace{0.01\textwidth}
    \hfill
    \begin{subfigure}{0.24\textwidth}
    \centering
    \input{Figs/results/success_rate/pushing_success}
    \end{subfigure}
    % \hspace{0.01\textwidth}
    \hfill
    \begin{subfigure}{0.24\textwidth}
    \centering
    \input{Figs/results/success_rate/img_sorting_success}
    \end{subfigure}
    \\
    \centering
    \begin{subfigure}{0.24\textwidth}
    \centering
    \input{Figs/results/entropy/avoiding_entropy}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
    \centering
    \input{Figs/results/entropy/aligning_entropy}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
    \centering
    \input{Figs/results/entropy/pushing_entropy}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
    \centering
    \input{Figs/results/entropy/img_sorting_entropy}
    \end{subfigure}
    \caption{Distillation performance from 4 \acrshort{lfd} tasks from D3IL datasets are demonstarted, where the red lines are the performance of \textcolor{red}{original continous diffusion model} and the blue lines are performance of \textcolor{blue}{original discrete diffusion model}. The results show \acrshort{method} is able to consistently replicate the performance of the original diffusion models.}
    \label{fig:distillation_1}
\end{figure}

==> Figs/distillation_2.tex <==
\begin{figure}[!t]
    \scriptsize
    \centering
    \sloppy
    \begin{subfigure}{0.24\textwidth}
    \centering
    \input{Figs/results/success_rate/stacking_1_success}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
    \centering
    \input{Figs/results/success_rate/stacking_2_success}
    \end{subfigure}
    % \hspace{0.01\textwidth}
    \hfill
    \begin{subfigure}{0.24\textwidth}
    \centering
    \input{Figs/results/success_rate/img_stacking_success}
    \end{subfigure}
    % \hspace{0.01\textwidth}
    \hfill
    \begin{subfigure}{0.24\textwidth}
    \centering
    \input{Figs/results/success_rate/block_push_success}

    \end{subfigure}
    \\
    \centering
    \begin{subfigure}{0.24\textwidth}
    \centering
    \input{Figs/results/entropy/stacking_1_entropy}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
    \centering
    \input{Figs/results/entropy/stacking_2_entropy}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
    \centering
    \input{Figs/results/entropy/img_stacking_entropy}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
    \centering
    \input{Figs/results/success_rate/kitchen_success}
    \end{subfigure}
    \caption{
    \todo{In this figure, we demonstrate the performance of }}
    \label{fig:distillation_2}
\end{figure}

==> Figs/results/backup/avoiding_entropy.tex <==
\begin{tikzpicture}
    \begin{axis}[
        ybar,
        ymin=0, ymax=1,
        % ylabel={Success Rate},
        % xlabel={Methods},
        xticklabels={D1, CM, VDD},
        % symbolic x coords = {D1, CM, VDD},
        % xtick=data,
        xtick={1, 2, 3},
        % xticklabels=\empty,
        xtick align=inside,
        % nodes near coords,
        error bars/.cd,
        % y dir=both, y explicit,
        grid=major,
        enlarge x limits=1.,
        width=1.3\textwidth,
        % title={Avoiding}
    ]
    % Data for bar graph
    \addplot[ybar, draw=none, fill=D1color, error bars/.cd, y dir=both, y explicit]coordinates {(1.45, 0.3) += (0,0.05) -= (0,0.05)};
    \addplot[ybar, draw=none, fill=CMcolor, error bars/.cd, y dir=both, y explicit]coordinates {(2, 0.4) += (0,0.05) -= (0,0.05)};
    \addplot[ybar, draw=none, fill=VDDcolor, error bars/.cd, y dir=both, y explicit]coordinates {(2.55, 0.6) += (0,0.05) -= (0,0.05)};
    
    % Expert success rate as a gray dashed horizontal line
    \draw[red, dashed, thick] 
        (rel axis cs:0,0.8) -- (rel axis cs:1,0.8);
    
    % Add a legend
    % \legend{Success Rate, Expert Success Rate}
    \end{axis}
\end{tikzpicture}

==> Figs/results/backup/avoiding_success_rate.tex <==
\begin{tikzpicture}
    \begin{axis}[
        ybar,
        ymin=0, ymax=1,
        % ylabel={Success Rate},
        % xlabel={Methods},
        xticklabels={D1, CM, VDD},
        % symbolic x coords = {D1, CM, VDD},
        % xtick=data,
        xtick={1, 2, 3},
        % xticklabels=\empty,
        xtick align=inside,
        % nodes near coords,
        error bars/.cd,
        % y dir=both, y explicit,
        grid=major,
        enlarge x limits=1.,
        width=1.3\textwidth,
        title={Avoiding}
    ]
    % Data for bar graph
    \addplot[ybar, draw=none, fill=D1color, error bars/.cd, y dir=both, y explicit]coordinates {(1.45, 0.84)};
    \addplot[ybar, draw=none, fill=CMcolor, error bars/.cd, y dir=both, y explicit]coordinates {(2, 0.4) += (0,0.05) -= (0,0.05)};
    \addplot[ybar, draw=none, fill=VDDcolor, error bars/.cd, y dir=both, y explicit]coordinates {(2.55, 0.95) += (0,0.01) -= (0,0.01)};
    
    % Expert success rate as a gray dashed horizontal line
    \draw[red, dashed, thick] 
        (rel axis cs:0,0.96) -- (rel axis cs:1,0.96);
    
    % Add a legend
    % \legend{Success Rate, Expert Success Rate}
    \end{axis}
\end{tikzpicture}

==> Figs/simulations/sim_tasks.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=\textwidth]{Figs/simulations/fig/sim7.png}
    \caption{We evaluate our model in the following simulated robot tasks. From left to right: Relay Kitchen \cite{gupta2019relay}, XArm Block Push \cite{florence2022implicit}, and five D3IL \cite{jia2024towards} tasks with rich behaviour diversities: Avoiding, Aligning, Pushing, Sorting and Stacking.}
    \label{fig:sim_tasks}
\end{figure}

==> Figs/vdd_algobox.tex <==
\begin{wrapfigure}{r}{0.55\textwidth} % 'r' for right, '0.5\textwidth' for width
  \vspace{-20pt} % Adjust vertical spacing as needed
  \begin{minipage}{0.55\textwidth}
    \begin{algorithm}[H]
      \caption{\acrfull{method}}
      \begin{algorithmic}[1]
        \REQUIRE Observation $S$, Actions $A$, pretrained denoising score function $s^\theta(s,a)$
        \STATE Initialize \acrshort{moe}: $\moe = \sum_{\comp} \gating \expert$
        \FOR{each iteration $i = 1, 2, \ldots, N$}
          % \FOR{each components update step $j=1,2, \ldots, M$}
            \STATE \textbf{Update Experts:}
            \STATE update $\expert$ with \todo{ref eq}
          % \ENDFOR
          % \FOR{each gating update step $k=1,2, \ldots, K$}
            \STATE \textbf{Update Gating:}
            \STATE compute gating targets with \eqref{eq:e_step}
            \STATE update $\gating$ using Cross Entropy loss
          % \ENDFOR
        \ENDFOR
        \STATE Output learned \acrshort{moe} $q^{\phi}(a|s)$
      \end{algorithmic}
    \end{algorithm}
  \end{minipage}
\end{wrapfigure}

==> Figs/vdd_inference.tex <==
\begin{wrapfigure}{r}{0.55\textwidth} % 'r' for right, '0.5\textwidth' for width
  \vspace{-20pt} % Adjust vertical spacing as needed
  \begin{minipage}{0.55\textwidth}
    \begin{algorithm}[H]
      \caption{\acrshort{method} Inference}
      \begin{algorithmic}[1]
        \REQUIRE Observation $s$
        \STATE Predict $\mu_{1...k}$, \text{Categorical(z)} in one forward pass.
        \STATE Sample a component $z \sim \text{Categorical}(z)$
        \STATE Select a = $\mu_z$
        \STATE \textbf{Return} $a$
      \end{algorithmic}
    \end{algorithm}
  \end{minipage}
\end{wrapfigure}

==> Rebuttals/arch_fig/arch.tex <==
% \renewcommand{\topfraction}{0.}
% \renewcommand{\bottomfraction}{0.}
% \renewcommand{\textfraction}{0.}
% \renewcommand{\floatpagefraction}{0.}

\begin{figure}[H]  
  \centering    
  \begin{minipage}{0.60\textwidth}      
      \vspace{-3cm}
      \label{sample-table}
      \centering
      \resizebox{\textwidth}{!}{%
        % \renewcommand{\arraystretch}{1.5}        
        \scriptsize
      \begin{tabular}{llllllll}
        \toprule
        Num. of Experts &1 &2 &4 &8 &16 \\ %&32 \\
        \midrule
        Parameters\ ($\times 10^4$) &144.23   &144.45  &144.89 &145.76 &147.50 \\ %&150.99    \\
        Times/1k Iters\ ($s$) &64.48   &70.19  &74.62 &106.98 &166.54 \\ %&301.02    \\
        \bottomrule        
      \end{tabular}
      }
      \vspace{-2pt}
      \captionof{table}{Adding more experts does not significantly increase the number of neural network parameters or the training time. We conducted the evaluation on the state-based avoiding task, using a machine with an RTX 3070 GPU and an i7-13700 CPU. This result is due to the optimized network architecture of the VDD model, as shown in Figure \ref{fig:vdd_net}. Adding more experts will only increase the number of output linear layers, i.e., the mean and covariance nets, while the transformer backbone which contains most of the parameters remains unchanged.}          
  \end{minipage}
    \hfill
    % \hspace{0.8cm}
  \begin{minipage}[t]{0.33\textwidth}
    % \vspace{-10cm}
    \def\arrowblue{black!20!blue}
    \def\arrowred{red}
    \def\sca{0.9}
    \begin{tikzpicture}[
        rrnode_nn/.style={rectangle, draw, minimum size=7mm, rounded corners=1mm, scale=\sca},    
        rrnode_score/.style={
            rectangle, draw, minimum size=6mm, scale=\sca, color=\arrowblue, ultra thick,
            dashed, dash pattern=on 3pt off 2pt,
            },
        rrnode_vdd/.style={
            draw, % draw the node border
            rectangle, % shape of the node
            text width=2.6cm, % width of the node
            align=center, % center-align the text
            rounded corners=1mm,
            ultra thick,
            % font=\sffamily % font style
        },
        rrnode_destill/.style={
            % draw, % draw the node border
            % rectangle, % shape of the node
            % text width=3cm, % width of the node
            align=center, % center-align the text
            % rounded corners=1mm,
            % font=\sffamily % font style
        },        
    ]
        % \tiny
        \scriptsize
        \centering
        \hspace{-0.3cm}
        % Import figure
        \node (image) at (0,0) {\includegraphics[width=4.6cm]{Figs/vdd_net/fig/vdd_arch.png}};
            
        % OBS        
        \node[rrnode_destill] (obs0) [below left=-0.31cm and -0.66cm of image]{{$...$}};
        \node[rrnode_destill] (obs1) [right=0.22cm of obs0]{{$\bm{s}_{k-2}$}};
        \node[rrnode_destill] (obs2) [right=0.04cm of obs1]{{$\bm{s}_{k-1}$}};
        \node[rrnode_destill] (obs3) [right=0.17cm of obs2]{{$\bm{s}_{k}$}};

        % Number of expersts
        \node[rrnode_destill] (n_exp) [below right=-2.5cm and -1.45cm of image]{Number of \\Experts Z};


        % weights
        \node[rrnode_destill] (w) [above left=-1.03cm and -0.77cm of image]{$\bm{w}_{z}$};

        % mean
        \node[rrnode_destill] (mean) [below right=0.18cm and 0.57cm of w]{$\bm{\mu}_{z}$};

        % Sigma
        \node[rrnode_destill] (Sigma) [right=0.59cm of mean]{$\bm{\Sigma}_{z}$};
        
    \end{tikzpicture}
    \captionsetup{margin={-0.4cm,0cm}}
    \caption{VDD's architecture\\ (same as Figure 4 in Appendix A)} 
    \label{fig:vdd_net}
  \end{minipage}
  \hspace{-0.8cm}
  \vspace{-5cm}
\end{figure}

==> Rebuttals/ddpm_kitchen_block.tex <==
\begin{table}[h]
\resizebox{\textwidth}{!}{
\begin{tabular}{c|cc||cc|>{\columncolor{gray!30}}c>{\columncolor{gray!30}}c>{\columncolor{gray!30}}c}
\toprule
 & \textbf{DDPM} & \textbf{BESO} & \textbf{DDPM-1} &\textbf{BESO-1} & \textbf{CD} & \textbf{VDD-DDPM(ours)} & \textbf{VDD-BESO(ours)}
\\ \hline
\textbf{Kitchen} &\red{3.66} & $4.06$ & \red{0.05} & $\underline{4.02}$ & $\bm{3.87\pm0.05}$ &\red{$3.29\pm0.09$} &$3.85\pm0.10$\\
\textbf{Block Push} &\red{0.96} &$0.96$ & \red{0.09} & $\underline{0.94}$ & $0.89\pm0.05$ &\red{$\bm{0.93\pm0.03}$} &$0.91\pm0.03$\\
\bottomrule
\end{tabular}
}
\caption{This table presents new evaluation on DDPM and VDD-DDPM in franka kitchen and block push environments}
\end{table}

==> Rebuttals/ddpm_new_results.tex <==
\begin{table}[H]
    \centering
    % \tiny
    \scriptsize
    % \footnotesize
    \setlength{\aboverulesep}{0pt}
    \setlength{\belowrulesep}{0pt}
    \renewcommand{\arraystretch}{1.5}        
    \begin{subtable}[t]{0.48\linewidth}
        \centering
        \input{Rebuttals/ddpm_only_new}
        \caption{Success Rate}
        \label{tab:ddpm_success}
    \end{subtable}
    % \\
    \hfill
    \begin{subtable}[t]{0.48\linewidth}
        \centering
        \input{Rebuttals/ddpm_training_time}
        \caption{Training Time (in Minutes)}
        \label{tab:ddpm_training}
    \end{subtable}
    \vspace{-0.15cm}
    \caption{
    New evaluation on DDPM and VDD-DDPM in Franka kitchen and block push environments, (a) VDD achieves $>96 \%$ performance of the original DDPM models in both tasks, (b) the training times were evaluated on a machine with an RTX 3070 GPU.
    } 
    % In most tasks \acrshort{method} achieves both high success rate and entropy.}
    \label{tab:ddpm_performance}
    \renewcommand{\arraystretch}{1}
    \vspace{-0.25cm}
\end{table}


==> Rebuttals/ddpm_only_new.tex <==
% \begin{table}[H]
\centering
    \setlength{\aboverulesep}{0pt}
    \setlength{\belowrulesep}{0pt}
    \renewcommand{\arraystretch}{1.5}        
    \scriptsize
% \resizebox{0.6\textwidth}{!}{
\scalebox{0.85}[1.0]{
\begin{tabular}{c|cc||>{\columncolor{gray!30}}c>{\columncolor{gray!30}}c}
\toprule
 & \textbf{DDPM} &\textbf{DDPM-1} &\textbf{VDD-DDPM(ours)} & \textbf{Percentage}
\\ \hline
\textbf{Kitchen} &3.35 & 0.22 &$3.24\pm0.12$ & $96.7\ \%$ \\
\textbf{Block Push} &0.96 &0.09 &$0.93\pm0.03$ & $96.9\ \%$\\
\bottomrule
\end{tabular}
}
% \caption{New evaluation on DDPM and VDD-DDPM in franka kitchen and block push environments.}
% \end{table}


==> Rebuttals/ddpm_training_time.tex <==
% \begin{table}[H]
\centering
    \setlength{\aboverulesep}{0pt}
    \setlength{\belowrulesep}{0pt}
    \renewcommand{\arraystretch}{1.5}        
    \scriptsize
% \resizebox{0.6\textwidth}{!}{
\scalebox{0.85}[1.0]{
\begin{tabular}{c|ccc}
\toprule
 & \textbf{DDPM} &\textbf{VDD-DDPM} & $\Sigma$\\ \hline
\textbf{Kitchen} &17 &70 & 87\\
\textbf{Block Push} &33 &95 & 128\\
\bottomrule
\end{tabular}
}
% \caption{New evaluation on DDPM and VDD-DDPM in franka kitchen and block push environments.}
% \end{table}


==> Rebuttals/table/destill_entropy.tex <==
% \begin{table}[!t]
% \centering
\scalebox{0.85}[1.0]{
\begin{tabular}{c|cc||>{\columncolor{gray!30}}c>{\color{red}\columncolor{gray!30}}c>{\columncolor{gray!30}}c>{\columncolor{gray!30}}c}
\toprule
                          & \textbf{BESO} &\textbf{BESO-1}            &  \textbf{CD}       & \textbf{CTM}                   & \textbf{VDD(ours)} \\ \hline
\textbf{Avoid}            & $0.87$        & $0.76$                    & $0.72\pm0.02$      & \underline{$\bm{0.79\pm0.04}$} & $0.72\pm0.12$\\
\textbf{Align}            & $0.67$        & $0.34$                    & $0.32\pm0.14$      & $0.31\pm0.28$                  & \underline{\bm{$0.40\pm0.04$}}\\
\textbf{Push}             & $0.76$        & $0.50$                    & $0.53\pm0.07$      & $0.54\pm0.08$                  & \underline{$\bm{0.69\pm0.08}$}\\
\textbf{Stack-1}          & $0.30$        & $\underline{0.26}$        & $\bm{0.19\pm0.12}$ & $0.18\pm0.08$                  & $0.16\pm0.03$\\
\textbf{Stack-2}          & $0.13$        & $0.07$                    & $0.03\pm0.05$      & $0.09\pm0.06$                  & \underline{$\bm{0.13\pm0.06}$}\\
\textbf{Sort-I}           & $0.19$        & $0.14$                    & $0.14\pm0.06$      & $0.08\pm0.05$                  & \underline{$\bm{0.22\pm0.03}$}\\
\textbf{Stack-I}          & $0.15$        & $0.10$                    & $0.06\pm0.01$      & $0.04\pm0.04$                  & \underline{$\bm{0.11\pm0.03}$}\\
\bottomrule
\end{tabular}
}
% \vspace{10pt}
% \caption{Distillation Entropy}
% \end{table}




% \begin{tabular}{c|cc||cc|>{\columncolor{gray!30}}c>{\columncolor{gray!30}}c>{\columncolor{gray!30}}c}
% \toprule
%                           & \textbf{DDPM} & \textbf{BESO} & \textbf{DDPM-1} &\textbf{BESO-1}            & \textbf{CD}       & \textbf{VDD-DDPM(ours)} & \textbf{VDD-BESO(ours)} \\ \hline
% \textbf{Avoiding}         &$0.90\pm0.02$  & $0.86\pm0.02$ & $0.38\pm0.05$   & $0.69\pm0.07$             &$\bm{0.72\pm0.02}$ & $0.37\pm0.01$      & $\bm{0.72\pm0.12}$\\
% \textbf{Aligning}         &$0.69\pm0.05$  & $0.72\pm0.04$ & $0.00\pm0.00$   & $0.24\pm0.08$             & $0.32\pm0.14$     & $0.25\pm0.09$      & \underline{\bm{$0.40\pm0.04$}}\\
% \textbf{Pushing}          &$0.76\pm0.04$  & $0.78\pm0.02$ & $0.00\pm0.00$   & $0.59\pm0.07$             &$0.53\pm0.07$      & $0.66\pm0.05$      & \underline{$\bm{0.69\pm0.08}$}\\
% \textbf{Stacking-1}       &$0.16\pm0.05$  & $0.34\pm0.04$ & $0.00\pm0.00$   & \underline{$0.28\pm0.03$} &$\bm{0.19\pm0.12}$ & $\bm{0.19\pm0.05}$ & $0.16\pm0.03$\\
% \textbf{Stacking-2}       &$0.10\pm0.02$  & $0.17\pm0.04$ & $0.00\pm0.00$   & $0.07\pm0.04$             &$0.03\pm0.05$      & $0.07\pm0.04$      & \underline{$\bm{0.13\pm0.06}$}\\
% \textbf{Sorting (Image)}  &$0.19\pm0.01$  & $0.22\pm0.02$ & $0.16\pm0.05$   & $0.16\pm0.02$             &$0.14\pm0.06$      & $0.12\pm0.03$      & \underline{$\bm{0.22\pm0.03}$}\\
% \textbf{Stacking (Image)} &$0.28\pm0.05$  & $0.14\pm0.04$ & $0.00\pm0.00$   & $0.12\pm0.02$             &$0.06\pm0.01$      & $0.05\pm0.02$      & \underline{$\bm{0.11\pm0.03}$}\\
% \bottomrule
% \end{tabular}

==> Rebuttals/table/destill_success.tex <==
% \begin{table}[!t]
% \centering
% \renewcommand{\arraystretch}{1.2}
\scalebox{0.85}[1.0]{
\begin{tabular}{c|cc||>{\columncolor{gray!30}}c>{\color{red}\columncolor{gray!30}}c>{\columncolor{gray!30}}c>{\columncolor{gray!30}}c}
\toprule
                            & \textbf{BESO}   & \textbf{BESO-1} & \textbf{CD}                      & \textbf{CTM}    & \textbf{VDD(ours)}       \\ \hline
\textbf{Avoid}              & $0.96$   & $0.84$   & $0.82\pm0.05$                  & $0.93\pm0.02$ & $\bm{\underline{0.95\pm0.01}}$\\
\textbf{Align}              & $0.85$   & $0.93$   & $\bm{\underline{0.94\pm0.08}}$ & $0.81\pm0.11$ & $0.86\pm0.04$\\
\textbf{Push}               & $0.78$   & $0.70$   & $0.66\pm0.05$                  & $0.80\pm0.07$ & $\underline{\bm{0.85\pm0.02}}$\\
\textbf{Stack-1}            & $0.91$   & $0.75$   & $0.69\pm0.06$                  & $0.54\pm0.17$ & $\underline{\bm{0.85\pm0.02}}$\\
\textbf{Stack-2}            & $0.70$   & $0.53$   & $0.46\pm0.11$                  & $0.30\pm0.09$ & $\underline{\bm{0.57\pm0.06}}$\\
\textbf{Sort-I}             & $0.70$   & $0.68$   & $0.71\pm0.07$                  & $0.70\pm0.07$ & $\underline{\bm{0.76\pm0.04}}$\\
\textbf{Stack-I}            & $0.66$   & $0.58$   & $\underline{\bm{0.63\pm0.01}}$ & $0.59\pm0.10$ & $0.60\pm0.04$ \\
\bottomrule
\end{tabular}
}
% \vspace{10pt}
% \caption{Results comparison between \acrshort{method} and SoTA \acrshort{moe} training approaches. The results suggest \acrshort{method} consistently outperform EM and IMC in terms of both precision and behaviour versatility.}
% \end{table}



% \begin{tabular}{c|cc||cc|>{\columncolor{gray!30}}c>{\columncolor{gray!30}}c>{\columncolor{gray!30}}c}
% \toprule
%                             & \textbf{DDPM} & \textbf{BESO}   & \textbf{DDPM-1} & \textbf{BESO-1} & \textbf{CD}                    & \textbf{VDD-DDPM(ours)}        & \textbf{VDD-BESO(ours)}
% \\ \hline
% \textbf{Avoiding}           &$0.93\pm0.02$  & $0.95\pm0.02$   & $0.06\pm0.01$   & $0.82\pm0.04$   & $0.82\pm0.05$                  & $0.92\pm0.02$                  & $\bm{\underline{0.95\pm0.01}}$\\
% \textbf{Aligning}           &$0.87\pm0.01$  & $0.85\pm0.01$   & $0.00\pm0.00$   & $0.92\pm0.01$   & $\bm{\underline{0.94\pm0.08}}$ & $0.70\pm0.07$                  & $0.86\pm0.04$\\
% \textbf{Pushing}            &$0.82\pm0.06$  & $0.79\pm0.02$   & $0.00\pm0.00$   & $0.69\pm0.09$   & $0.66\pm0.05$                  & $0.61\pm0.04$                  & $\underline{\bm{0.85\pm0.02}}$\\
% \textbf{Stacking-1}         &$0.87\pm0.03$  & $0.91\pm0.02$   & $0.00\pm0.00$   & $0.79\pm0.05$   & $0.69\pm0.06$                  & $0.81\pm0.08$                  & $\underline{\bm{0.85\pm0.02}}$\\
% \textbf{Stacking-2}         &$0.69\pm0.03$  & $0.71\pm0.01$   & $0.00\pm0.00$   & $0.51\pm0.01$   & $0.46\pm0.11$                  & $\underline{\bm{0.60\pm0.07}}$ & $0.57\pm0.06$\\
% \textbf{Sorting (Image)}    &$0.75\pm0.03$  & $0.77\pm0.01$   & $0.39\pm0.14$   & $0.77\pm0.02$   & $0.71\pm0.07$                  & $\underline{\bm{0.80\pm0.04}}$ & $0.76\pm0.04$\\
% \textbf{Stacking (Image)}   &$0.66\pm0.04$  & $0.62\pm0.08$   & $0.00\pm0.00$   & $0.56\pm0.06$   & $0.63\pm0.01$                  & $\underline{\bm{0.78\pm0.02}}$ & $0.60\pm0.04$ \\
% \bottomrule
% \end{tabular}

==> Rebuttals/table/distillation.tex <==
\begin{table}[H]
    \centering
    % \tiny
    \scriptsize
    % \footnotesize
    \setlength{\aboverulesep}{0pt}
    \setlength{\belowrulesep}{0pt}
    \renewcommand{\arraystretch}{1.5}        
    \begin{subtable}[t]{0.48\linewidth}
        \centering
        \input{Rebuttals/table/destill_success}
        \caption{Task Success Rate}
        \label{tab:distill_success}
    \end{subtable}
    % \\
    \hfill
    \begin{subtable}[t]{0.48\linewidth}
        \centering
        \input{Rebuttals/table/destill_entropy}
        \caption{Task Entropy}
        \label{tab:distill_entropy}
    \end{subtable}
    \vspace{-0.15cm}
    \caption{Comparison of distillation performance, (a) \acrshort{method} achieves on-par performance with Consistency Distillation (CD) and Consistency Trajectory Model (CTM, newly added, shown in {\color{red}{red}}) (b) \acrshort{method} is able to possess versatile skills (indicated by high task entropy) while keeping high success rate. The \textbf{best results} for distillation are bolded, and the \underline{highest values} except origin models are underlined. All three distilled models share the same transformer backbone.} 
    % In most tasks \acrshort{method} achieves both high success rate and entropy.}
    \label{tab:distill_performance}
    \renewcommand{\arraystretch}{1}
    \vspace{-0.25cm}
\end{table}


==> Rebuttals/trainingXcmps.tex <==
\begin{table}[h]
  \label{sample-table}
  \centering
  \resizebox{0.6\textwidth}{!}{%
  \begin{tabular}{llllllll}
    \toprule
    Num. of Experts &1 &2 &4 &8 &16 \\ %&32 \\
    \midrule
    Parameters\ ($\times 10^4$) &144.23   &144.45  &144.89 &145.76 &147.50 \\ %&150.99    \\
    Times/1k Iters\ ($s$) &64.48   &70.19  &74.62 &106.98 &166.54 \\ %&301.02    \\
    \bottomrule
  \end{tabular}
  }
  \vspace{-2pt}
  \caption{This table presents how the number of network parameters and training time scale with the number of experts. We conducted the evaluation in the state-based avoiding task with 4 layers of shared transformer blocks and a training batch size of $1024$. All the evaluations are conducted on the same machine with RTX 3070 GPU and i7-13700 CPU. }
\end{table}


==> Tables/distillation_entropy.tex <==
% \begin{table}[!t]
% \centering
\resizebox{\textwidth}{!}{
\begin{tabular}{c|cc||cc|>{\columncolor{gray!30}}c>{\columncolor{gray!30}}c>{\columncolor{gray!30}}c}
\toprule
 & \textbf{DDPM} & \textbf{BESO} & \textbf{DDPM-1} &\textbf{BESO-1} & \textbf{CD} & \textbf{VDD-DDPM(ours)} & \textbf{VDD-BESO(ours)}
\\ \hline
\textbf{Avoiding} &$0.90\pm0.02$ & $0.86\pm0.02$ & $0.38\pm0.05$ & $0.69\pm0.07$ &$\bm{0.72\pm0.02}$ &$0.37\pm0.01$ &$\bm{0.72\pm0.12}$\\
\textbf{Aligning} &$0.69\pm0.05$ & $0.72\pm0.04$ & $0.00\pm0.00$ & $0.24\pm0.08$ & $0.32\pm0.14$ &$0.25\pm0.09$ &\underline{\bm{$0.40\pm0.04$}}\\
\textbf{Pushing} &$0.76\pm0.04$ & $0.78\pm0.02$ & $0.00\pm0.00$ & $0.59\pm0.07$ &$0.53\pm0.07$ &$0.66\pm0.05$ &\underline{$\bm{0.69\pm0.08}$}\\
\textbf{Stacking-1} &$0.16\pm0.05$ &$0.34\pm0.04$ &$0.00\pm0.00$ &\underline{$0.28\pm0.03$} &$\bm{0.19\pm0.12}$ &$\bm{0.19\pm0.05}$ &$0.16\pm0.03$\\
\textbf{Stacking-2} &$0.10\pm0.02$ & $0.17\pm0.04$ &$0.00\pm0.00$ &$0.07\pm0.04$ &$0.03\pm0.05$ &$0.07\pm0.04$ &\underline{$\bm{0.13\pm0.06}$}\\
\textbf{Sorting (Image)} &$0.19\pm0.01$ &$0.22\pm0.02$ &$0.16\pm0.05$ &$0.16\pm0.02$ &$0.14\pm0.06$ &$0.12\pm0.03$ & \underline{$\bm{0.22\pm0.03}$}\\
\textbf{Stacking (Image)} &$0.28\pm0.05$ &$0.14\pm0.04$ &$0.00\pm0.00$ &$0.12\pm0.02$ &$0.06\pm0.01$ &$0.05\pm0.02$ &\underline{$\bm{0.11\pm0.03}$}\\
% \textbf{Kitchen} &- & $4.06$ & - & $4.02$ & $\bm{3.87\pm0.05}$ &- &$3.85\pm0.10$\\
% \textbf{Block Push} &- &$0.96$ & - & $0.94$ & $0.89\pm0.05$ &- &$\bm{0.91\pm0.03}$\\
\bottomrule
\end{tabular}
}
% \vspace{10pt}
% \caption{Distillation Entropy}
% \end{table}

==> Tables/distillation_entropy_old.tex <==
% \begin{table}[!t]
% \centering
% \resizebox{0.5\textwidth}{!}{
\begin{tabular}{c|cc||cc|>{\columncolor{gray!30}}c>{\columncolor{gray!30}}c>{\columncolor{gray!30}}c}
\toprule
 & \textbf{DDPM} & \textbf{BESO} & \textbf{DDPM-1} &\textbf{BESO-1} & \textbf{CD} & \textbf{VDD-DDPM(ours)} & \textbf{VDD-BESO(ours)}
\\ \hline
\textbf{Avoiding} &$0.89$ & $0.87$ & $0.25$ & $\underline{0.76}$ &$\bm{0.72\pm0.02}$ &$0.37\pm0.01$ &$\bm{0.72\pm0.12}$\\
\textbf{Aligning} &$0.62$ & $0.67$ & $0.00$ & $0.34$ & $0.32\pm0.14$ &$0.25\pm0.09$ &\underline{\bm{$0.40\pm0.04$}}\\
\textbf{Pushing} &$0.74$ & $0.76$ & $0.00$ & $0.50$ &$0.53\pm0.07$ &$0.66\pm0.05$ &\underline{$\bm{0.69\pm0.08}$}\\
\textbf{Stacking-1} &$0.24$ &$0.30$ &$0.00$ &\underline{$0.26$} &$\bm{0.19\pm0.12}$ &$\bm{0.19\pm0.05}$ &$0.16\pm0.03$\\
\textbf{Stacking-2} &$0.12$ &$0.13$ &$0.00$ &$0.07$ &$0.03\pm0.05$ &$0.07\pm0.04$ &\underline{$\bm{0.13\pm0.06}$}\\
\textbf{Sorting (Image)} &$0.16$ &$0.19$ &$0.09$ &$0.14$ &$0.14\pm0.06$ &$0.12\pm0.03$ & \underline{$\bm{0.22\pm0.03}$}\\
\textbf{Stacking (Image)} &$0.31$ &$0.15$ &$0.00$ &$0.10$ &$0.06\pm0.01$ &$0.05\pm0.02$ &\underline{$\bm{0.11\pm0.03}$}\\

\bottomrule
\end{tabular}
% }
% \vspace{10pt}
% \caption{Distillation Entropy}
% \end{table}

==> Tables/distillation_success.tex <==
% \begin{table}[!t]
% \centering
% \renewcommand{\arraystretch}{1.5}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|cc||cc|>{\columncolor{gray!30}}c>{\columncolor{gray!30}}c>{\columncolor{gray!30}}c}
\toprule
 & \textbf{DDPM} & \textbf{BESO} & \textbf{DDPM-1} &\textbf{BESO-1} & \textbf{CD} & \textbf{VDD-DDPM(ours)} & \textbf{VDD-BESO(ours)}
\\ \hline
\textbf{Kitchen} &- & $3.98\pm0.07$ & - & $\underline{3.92\pm0.15}$ & $\bm{3.87\pm0.05}$ &- &$3.85\pm0.10$\\
\textbf{Block Push} &- &$0.96\pm0.02$ & - & $0.90\pm0.01$ & $0.89\pm0.05$ &- &$\underline{\bm{0.91\pm0.03}}$\\
\hline
\textbf{Avoiding} &$0.93\pm0.02$ & $0.95\pm0.02$ & $0.06\pm0.01$ & $0.82\pm0.04$ &$0.82\pm0.05$ &$0.92\pm0.02$ &$\bm{\underline{0.95\pm0.01}}$\\
\textbf{Aligning} &$0.87\pm0.01$ & $0.85\pm0.01$ & $0.00\pm0.00$ & $0.92\pm0.01$ &$\bm{\underline{0.94\pm0.08}}$ &$0.70\pm0.07$ &$0.86\pm0.04$\\
\textbf{Pushing} &$0.82\pm0.06$ & $0.79\pm0.02$ & $0.00\pm0.00$ & $0.69\pm0.09$ &$0.66\pm0.05$ &$0.61\pm0.04$ &$\underline{\bm{0.85\pm0.02}}$\\
\textbf{Stacking-1} &$0.87\pm0.03$ &$0.91\pm0.02$ &$0.00\pm0.00$ &$0.79\pm0.05$ &$0.69\pm0.06$ &$0.81\pm0.08$ & $\underline{\bm{0.85\pm0.02}}$\\
\textbf{Stacking-2} &$0.69\pm0.03$ &$0.71\pm0.01$ &$0.00\pm0.00$ &$0.51\pm0.01$ &$0.46\pm0.11$ &$\underline{\bm{0.60\pm0.07}}$ &$0.57\pm0.06$\\
\textbf{Sorting (Image)} &$0.75\pm0.03$ &$0.77\pm0.01$ &$0.39\pm0.14$ &$0.77\pm0.02$ &$0.71\pm0.07$ &$\underline{\bm{0.80\pm0.04}}$ & $0.76\pm0.04$\\
\textbf{Stacking (Image)} &$0.66\pm0.04$ &$0.62\pm0.08$ &$0.00\pm0.00$ &$0.56\pm0.06$ &$0.63\pm0.01$ &$\underline{\bm{0.78\pm0.02}}$ &$0.60\pm0.04$ \\
\bottomrule
\end{tabular}


}
% \vspace{10pt}
% \caption{Results comparison between \acrshort{method} and SoTA \acrshort{moe} training approaches. The results suggest \acrshort{method} consistently outperform EM and IMC in terms of both precision and behaviour versatility.}
% \end{table}



==> Tables/distillation_success_old.tex <==
% \begin{table}[!t]
% \centering
% \renewcommand{\arraystretch}{1.5}
% \resizebox{0.48\textwidth}{!}{
\begin{tabular}{c|cc||cc|>{\columncolor{gray!30}}c>{\columncolor{gray!30}}c>{\columncolor{gray!30}}c}
\toprule
 & \textbf{DDPM} & \textbf{BESO} & \textbf{DDPM-1} &\textbf{BESO-1} & \textbf{CD} & \textbf{VDD-DDPM(ours)} & \textbf{VDD-BESO(ours)}
\\ \hline
\textbf{Kitchen} &- & $4.06$ & - & $\underline{4.02}$ & $\bm{3.87\pm0.05}$ &- &$3.85\pm0.10$\\
\textbf{Block Push} &- &$0.96$ & - & $\underline{0.94}$ & $0.89\pm0.05$ &- &$\underline{\bm{0.91\pm0.03}}$\\
\hline
\textbf{Avoiding} &$0.94$ & $0.96$ & $0.09$ & $0.84$ &$0.82\pm0.05$ &$0.92\pm0.02$ &$\bm{\underline{0.95\pm0.01}}$\\
\textbf{Aligning} &$0.85$ & $0.85$ & $0.00$ & $0.93$ &$\bm{\underline{0.94\pm0.08}}$ &$0.70\pm0.07$ &$0.86\pm0.04$\\
\textbf{Pushing} &$0.74$ & $0.78$ & $0.00$ & $0.70$ &$0.66\pm0.05$ &$0.61\pm0.04$ &$\underline{\bm{0.85\pm0.02}}$\\
\textbf{Stacking-1} &$0.89$ &$0.91$ &$0.00$ &$0.75$ &$0.69\pm0.06$ &$0.81\pm0.08$ & $\underline{\bm{0.85\pm0.02}}$\\
\textbf{Stacking-2} &$0.68$ &$0.70$ &$0.00$ &$0.53$ &$0.46\pm0.11$ &$\underline{\bm{0.60\pm0.07}}$ &$0.57\pm0.06$\\
\textbf{Sorting (Image)} &$0.69$ &$0.70$ &$0.20$ &$0.68$ &$0.71\pm0.07$ &$\underline{\bm{0.80\pm0.04}}$ & $0.76\pm0.04$\\
\textbf{Stacking (Image)} &$0.58$ &$0.66$ &$0.00$ &$0.58$ &$0.63\pm0.01$ &$\underline{\bm{0.78\pm0.02}}$ &$0.60\pm0.04$ \\
\bottomrule
\end{tabular}
% }
% \vspace{10pt}
% \caption{Results comparison between \acrshort{method} and SoTA \acrshort{moe} training approaches. The results suggest \acrshort{method} consistently outperform EM and IMC in terms of both precision and behaviour versatility.}
% \end{table}



==> Tables/inference_time.tex <==
\begin{table}
  \label{sample-table}
  \centering
  \begin{tabular}{llllllll}
    \toprule
    % \multicolumn{2}{c}{Method}                   \\
    % \cmidrule(r){1-2}
    NFE &1 &4 &$\bm{8}$ &16 &32 &64 \\
    \midrule
    Cont. Diffusion &3.96   &6.79  &$\bm{10.17}$ &17.27 &31.72 &59.73    \\
    Disc. Diffusion &2.17   &5.02  &$\bm{8.48}$ &15.56 &31.05 &60.34     \\
    \textbf{\acrshort{method} (Ours)}     & \bf{2.09}  \\
    \bottomrule
  \end{tabular}
  \vspace{10pt}
  \caption{Inference times for state-based avoiding, expressed in milliseconds, between \acrshort{method} and Diffusion models over various denoising steps.}
\end{table}


==> Tables/inference_time_image_stacking.tex <==
% \begin{table}
%   \label{sample-table}
%   \centering
%   \renewcommand{\arraystretch}{1.25}
%   \begin{tabular}{cccc>{\columncolor{gray!30}}c}
%     \toprule
%     % \multicolumn{2}{c}{Method}                   \\
%     % \cmidrule(r){1-2}
%     NFE &1 &4 &8 &16 \rule{0pt}{4mm}\\
%     \hline
%     Cont. Diffusion &9.69   &12.72  &16.39 &23.68 \\
%     Disc. Diffusion &6.49   &9.33  &12.79 &19.90 \\
%     Consistency Model &? \\
%     \textbf{\acrshort{method} (Ours)}     & \bf{4.91}  \\
%     \bottomrule
%   \end{tabular}
%   \vspace{10pt}
%   \caption{Inference times for image-based stacking, expressed in milliseconds, between \acrshort{method} and Diffusion models over various denoising steps.}
% \end{table}

%%%%%%%%%%%%%%%%%%%
% \begin{wraptable}{r}{0.6\textwidth} % 'r' for right, 0.6\textwidth for width
%     \centering
%     \renewcommand{\arraystretch}{1.25}
%     \begin{tabular}{cccc>{\columncolor{gray!30}}c}
%         \toprule
%         NFE & 1 & 4 & 8 & 16 \rule{0pt}{4mm} \\
%         \hline
%         Cont. Diffusion & 9.69 & 12.72 & 16.39 & 23.68 \\
%         Disc. Diffusion & 6.49 & 9.33 & 12.79 & 19.90 \\
%         Consistency Model & ? & & & \\
%         \textbf{\acrshort{method} (Ours)} & \bf{4.91} & & & \\
%         \bottomrule
%     \end{tabular}
%     \vspace{10pt}
%     \caption{Inference times for image-based stacking, expressed in milliseconds, between \acrshort{method} and Diffusion models over various denoising steps.}
%     \label{sample-table}
% \end{wraptable}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{wraptable}{r}{0.5\textwidth} % 'r' for right, 0.6\textwidth for width
    \centering
    \scriptsize
    \renewcommand{\arraystretch}{1.25}
    \begin{tabular}{cccc>{\columncolor{gray!30}}c}
        \toprule
        NFE & 1 & 4 & 8 & 16 \rule{0pt}{4mm} \\
        \hline
        Cont. Diffusion & 9.69 & 12.72 & 16.39 & 23.68 \\
        Disc. Diffusion & 6.49 & 9.33 & 12.79 & 19.90 \\
        Consistency Model & ? & & & \\
        \textbf{\acrshort{method} (Ours)} & \bf{4.91} & & & \\
        \bottomrule
    \end{tabular}
    \vspace{10pt}
    \caption{Inference times for image-based stacking, expressed in milliseconds, between \acrshort{method} and Diffusion models over various denoising steps.}
    \label{sample-table}
\end{wraptable}

==> Tables/inference_time_state_pushing.tex <==
\begin{table}
  \label{sample-table}
  \centering
  \renewcommand{\arraystretch}{1.25}
  \begin{tabular}{cccccc>{\columncolor{gray!30}}c}
    \toprule
    % \multicolumn{2}{c}{Method}                   \\
    % \cmidrule(r){1-2}
    NFE &1 &4 &$\bm{8}$ &16 &32 &64 \\
    \hline
    Cont. Diffusion &4.03   &8.08  &10.38 &17.34 &32.14 &60.64    \\
    Disc. Diffusion &2.15   &4.90  &8.25 &14.89 &29.47 &55.62    \\
    Consistency Model &  $?$ \\
    \textbf{\acrshort{method} (Ours)}     & \bf{2.16}  \\
    \bottomrule
  \end{tabular}
  \vspace{10pt}
  \caption{Inference times for state-based pushing, expressed in milliseconds, between \acrshort{method} and Diffusion models over various denoising steps. Shaded region is the default setting for Diffusion models in this task.}
\end{table}


==> Tables/main_results.tex <==
% \begin{table}
%   \caption{Sample table title}
%   \label{sample-table}
%   \centering
%   \begin{tabular}{llllllll}
%     \toprule
%     \multicolumn{2}{c}{Part}                   \\
%     \cmidrule(r){1-2}
%     Name     & Description     & Size ($\mu$m) \\
%     \midrule
%     Franka Kitchen & Input terminal  & $\sim$100     \\
%     Block Push     & Output terminal & $\sim$10      \\
%     Soma     & Cell body       & up to $10^6$  \\
%     \bottomrule
%   \end{tabular}
% \end{table}

\begin{table}[ht]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
& \multicolumn{2}{c|}{\textbf{Avoiding}} & \multicolumn{2}{c|}{\textbf{Aligning}} & \multicolumn{2}{c|}{\textbf{Pushing}} \\ \hline
 \textbf{Algorithm} & \textbf{Success Rate} & \textbf{Entropy} & \textbf{Success Rate} & \textbf{Entropy} & \textbf{Success Rate} & \textbf{Entropy} \\ \hline
Disc. Diffusion & $0.94$ & $0.89$ & $0.85$ & $0.62$ & $0.74$ & $0.74$ \\ \hline
DD - 1 step & $0.09$ & $0.25$ & $0.00$ & $0.00$ & $0.00$ & $0.00$ \\ \hline
Cont. Diffusion & $0.96$ & $0.87$ & $0.85$ & $0.67$ & $0.78$ & $0.76$ \\ \hline
CD - 1 step & $0.84$ & $0.76$ & $0.91$ & $0.34$ & $0.70$ & $0.50$ \\ \hline
Consistency Model & $0.82\pm0.05$ & $0.72\pm0.02$ & $0.94\pm0.08$ & $0.32\pm0.14$ & $0.66\pm0.05$ & $0.53\pm0.07$ \\ \hline
EM-GPT & $0.65\pm0.18$ & $0.17\pm0.13$ & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.01\pm0,01$ & $0.00\pm0.00$ \\ \hline
IMC-GPT & $0.75\pm0.08$ & $0.82\pm0.05$ & $0.83\pm0.02$ & $0.27\pm0.09$ & $0.76\pm0.04$ & $0.31\pm0.03$ \\ \hline
% VPD-Gaussian   & X\% & $0.00\pm0.00$ & X\% & $0.00\pm0.00$ & X\% & $0.00\pm0.00$ \\ \hline
\textbf{VPD-DD (Ours)} & $0.92\pm0.02$ & $0.37\pm0.01$ &  $0.70\pm0.05$ & $0.25\pm0.09$ & $0.61\pm0.04$ & $0.66\pm0.05$ \\ \hline
\textbf{VPD-CD (Ours)}  & $0.95\pm0.01$ & $0.72\pm0.12$ & $0.86\pm0.04$ & $0.40\pm0.04$ & $0.85\pm0.02$ & $0.69\pm0.08$ \\ \hline
\hline
& \multicolumn{2}{c|}{\textbf{Stacking 1}} & \multicolumn{2}{c|}{\textbf{Stacking 2}} & \multicolumn{2}{c|}{\textbf{Kitchen}} \\ \hline
\textbf{Algorithm}  & \textbf{Success Rate} & \textbf{Entropy} & \textbf{Success Rate} & \textbf{Entropy} & \textbf{Reward} & \textbf{-} \\ \hline
Disc. Diffusion & $0.89$ & $0.24$ & $0.68$ & $0.12$ & - & - \\ \hline
DD - 1 step & $0.00$ & $0.00$ & $0.00$ & $0.00$ & - & - \\ \hline
Cont. Diffusion & $0.91$ & $0.30$ & $0.70$ & $0.13$ & $4.06$ & - \\ \hline
CD - 1 step & $0.75$ & $0.26$ & $0.53$ & $0.07$ & $4.02$ & - \\ \hline
Consistency Model & $0.68\pm0.06$ & $0.19\pm0.12$ & $0.46\pm0.11$ & $0.03\pm0.05$ & $3.87\pm0.05$\ & - \\ \hline
EM-GPT & $0.58\pm0.06$ & $0.43\pm0.08$ & $0.34\pm0.07$ & $0.27\pm0.05$ & $3.67\pm0.05$ & - \\ \hline
IMC-GPT & $0.54\pm0.05$ & $0.37\pm0.04$ & $0.29\pm0.07$ & $0.17\pm0.07$ & $3.62\pm0.10$ & - \\ \hline
% VPD-Gaussian   & X\% & Y & X\% & Y & X\% & - \\ \hline
\textbf{VPD-DD (Ours)} & X\% & Y & X\% & Y & - & - \\ \hline
\textbf{VPD-CD (Ours)}  & $0.83\pm0.09$ & $0.16\pm0.03$ & $0.57\pm0.06$ & $0.13\pm0.06$ & $3.85\pm0.10$ & - \\ \hline
\hline
& \multicolumn{2}{c|}{\textbf{Block Push}} & \multicolumn{2}{c|}{\textbf{Sorting (Image-based)}} & \multicolumn{2}{c|}{\textbf{Stacking (Image-based)}} \\ \hline
 \textbf{Algorithm} & \textbf{Reward} & \textbf{-} & \textbf{Success Rate} & \textbf{Entropy} & \textbf{Success Rate} & \textbf{Entropy} \\ \hline
Disc. Diffusion & - & - & $0.69$ & $0.16$ & $0.58$ & $0.31$ \\ \hline
DD - 1 step & - & - & $0.20$ & $0.09$ & $0.00$ & $0.00$ \\ \hline
Cont. Diffusion & $0.96$ & - & $0.70$ & $0.19$ & $0.66$ & $0.15$ \\ \hline
CD - 1 step & $0.94$ & - & $0.68$ & $0.14$ & $0.58$ & $0.10$ \\ \hline
Consistency Model & $0.89\pm0.05$ & - & $0.71\pm0.07$ & $0.14\pm0.06$ & $0.625\pm0.008$ & $0.056\pm0.003$ \\ \hline
EM-GPT & $0.88\pm0.04$ & - & $0.73\pm0.03$ & $0.11\pm0.01$ & X\% & Y \\ \hline
IMC-GPT & $0.89\pm0.04$ & - & $0.71\pm0.04$ & $0.14\pm0.03$ & X\% & Y \\ \hline
% VPD-Gaussian   & X\% & - & X\% & Y & X\% & Y \\ \hline
\textbf{VPD-DD (Ours)} & - & - & X\% & Y & $0.78\pm0.05$ & $0.08\pm0.02$ \\ \hline
\textbf{VPD-CD (Ours)}  & $0.91\pm0.03$ & - & $0.75\pm0.04$ & $0.17\pm0.02$ & $0.58\pm0.05$ & $0.12\pm0.02$ \\ \hline
\end{tabular}
}
\vspace{10pt}
\caption{Results of Different Algorithms on Various Datasets}
\end{table}

==> Tables/moe_results.tex <==
\begin{table}[!t]
\centering
\renewcommand{\arraystretch}{1.2}
\resizebox{\textwidth}{!}{
\begin{tabular}{ccccccccc}
\toprule
& \multicolumn{2}{c}{\textbf{EM-GPT}} & \multicolumn{2}{c}{\textbf{IMC-GPT}} & \multicolumn{2}{c}{\textbf{\acrshort{method}-DDPM (Ours)}} & \multicolumn{2}{c}{\textbf{VDD-BESO (Ours)}}\\ \hline
 \textbf{Environments} & \textbf{Success Rate} & \textbf{Entropy} & \textbf{Success Rate} & \textbf{Entropy} & \textbf{Success Rate} & \textbf{Entropy}  & \textbf{Success Rate} & \textbf{Entropy} \\ \hline
\textbf{Avoiding} & $0.65\pm0.18$ & $0.17\pm0.13$ & $0.75\pm0.08$ & $\bf{0.82\pm0.05}$ & $0.92\pm0.02$ & $0.37\pm0.01$ & $\bf{0.95\pm0.01}$ & $0.73\pm0.09$ \\ 
\textbf{Aligning} & $0.78\pm0.04$ & $0.38\pm0.11$ &  $0.83\pm0.02$ & $0.27\pm0.09$ & $0.70\pm0.07$ & $0.25\pm0.09$ & $\bf{0.86\pm0.04}$ & $\bm{0.40\pm0.04}$\\ 
\textbf{Pushing} & $0.16\pm0.07$ & $0.14\pm0.10$ & $0.76\pm0.04$ & $0.31\pm0.03$ & $0.61\pm0.04$ & $0.66\pm0.05$ & $\bf{0.85\pm0.02}$ & $\bf{0.69\pm0.08}$ \\ 
\textbf{Stacking-1}  & $0.58\pm0.06$ &$\bf{0.43\pm0.08}$ & $0.54\pm0.05$ & $0.37\pm0.04$ & $0.81\pm0.08$ & $0.19\pm0.05$ & $\bf{0.83\pm0.09}$ & $0.16\pm0.03$\\ 
\textbf{Stacking-2}  & $0.34\pm0.07$ & $\bm{0.27\pm0.05}$ & $0.29\pm0.07$ & $0.17\pm0.07$ & $\bm{0.60\pm0.07}$ & $0.07\pm0.04$ & $0.57\pm0.06$ & $0.13\pm0.06$\\ 
\textbf{Sorting (image)}  & $0.69\pm0.02$ & $0.13\pm0.03$ &$0.74\pm0.04$ & $0.10\pm0.03$ & $\bm{0.80\pm0.04}$ & $0.12\pm0.03$ &$0.76\pm0.03$ &$\bm{0.22\pm0.03}$\\ 
\textbf{Stacking (image)}  & $0.04\pm0.03$ & $0.00\pm0.00$ & $0.39\pm0.10$ & $0.05\pm0.04$ & $\bf{0.78\pm0.02}$ & $0.08\pm0.02$ & $0.60\pm0.04$ & $\bm{0.11\pm0.03}$\\ 
% \textbf{Stacking-2 (image)}  & $0.04\pm0.03$ & $0.00\pm0.00$ & $0.39\pm0.10$ & $0.05\pm0.04$ & $\bf{0.78\pm0.02}$ & $0.08\pm0.02$ & $0.58\pm0.05$ & $\bm{0.12\pm0.02}$\\ 
\textbf{Relay Kitchen}  & $3.62\pm0.10$ & - & $3.67\pm0.05$ & - & - & - &$\bf{3.85\pm0.10}$ & - \\ 
\textbf{Block Push}  & $0.88\pm0.04$ & - & $0.89\pm0.04$ & - & - & - & $\bm{0.91\pm0.03}$ & - \\
\bottomrule
\end{tabular}
}
\vspace{10pt}
\caption{Results comparison between \acrshort{method} and SoTA \acrshort{moe} training approaches. The results suggest \acrshort{method} consistently outperforms EM and IMC in terms of both precision and behavior versatility, measured by the task entropy. \red{A bit more information needed, like how many tasks are outperformed and in which margin ....}}
\label{tab:moe_results}
\vspace{-0.5cm}
\end{table}
% \vspace{-0.5cm}
\renewcommand{\arraystretch}{1}
